Deep Distributional Time Series Models and the Probabilistic Forecasting of Intraday Electricity Prices

Recurrent neural networks (RNNs) with rich feature vectors of past values can provide accurate point forecasts for series that exhibit complex serial dependence. We propose two approaches to constructing deep time series probabilistic models based on a variant of RNN called an echo state network (ESN). The first is where the output layer of the ESN has stochastic disturbances and a shrinkage prior for additional regularization. The second approach employs the implicit copula of an ESN with Gaussian disturbances, which is a deep copula process on the feature space. Combining this copula with a non-parametrically estimated marginal distribution produces a deep distributional time series model. The resulting probabilistic forecasts are deep functions of the feature vector and also marginally calibrated. In both approaches, Bayesian Markov chain Monte Carlo methods are used to estimate the models and compute forecasts. The proposed models are suitable for the complex task of forecasting intraday electricity prices. Using data from the Australian National Electricity Market, we show that our deep time series models provide accurate short term probabilistic price forecasts, with the copula model dominating. Moreover, the models provide a flexible framework for incorporating probabilistic forecasts of electricity demand as additional features, which increases upper tail forecast accuracy from the copula model significantly.

==> append.tex <==
%\newpage
%\appendix

\noindent

\section{}\label{app:postN}
This appendix provides the MCMC sampler for drawing from
the posterior of $\varthetavec=\lbrace\betavec,\sigma^2,\tau^2\rbrace$ in the Gaussian probabilistic 
ESN for a given configuration $\xivec$, and the algorithm for simulating draws from forecast distribution.

\noindent \underline{Algorithm~1} {\em (MCMC sampler for Gaussian probabilistic ESN)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
\setlength{\itemindent}{0.5cm}
\item[1.] Generate from $\betavec|\{\varthetavec\setminus\betavec\},X,\yvec$.
\item[2.] Generate from $\sigma^2|\{\varthetavec\setminus\sigma^2\},X,\yvec$.
\item[3.] Generate from $\tau^2|\{\varthetavec\setminus\tau^2\},X,\yvec$.%Perform MH-step for $\tau^2$
\end{itemize}

\noindent 
The conditional posteriors above are standard and their derivation is omitted here.
% At Step~1
%$\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$, with
% $\Sigma_{\beta}=(B_\xi(X)'B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$ and $\mu_{\beta}=\Sigma_{\beta}B_\xi(X)'\yvec/\sigma^2$. At Steps~2 and~3
% the distributions are inverse Gammas, where
%$\sigma^2\sim\mathcal{IG}(a+\frac{T}{2},b+\frac{1}{2}\varepsilonvec'\varepsilonvec)$
%and 
%$\tau^2 \sim\mathcal{IG}(\tilde a+\frac{p}{2},\tilde b+\frac{1}{2}\betavec'\betavec)$,
%with $p=\dim(\betavec)$. 
The scheme is very fast and
converges quickly. Accurate mixture estimates of the 
posterior mean $\hat{\varthetavec}=E(\varthetavec|X,\yvec)$ 
can be computed from a few hundred draws post-convergence.

Algorithm~2 below is used to simulate from the ensemble forecast distribution
at~(5). Let 
$y^r_{i,t}$ denote the $i$th Monte Carlo draw of (logarithmic) price
in region $r\in\{1,2,\ldots,5\}$ at time $t$. For time points $t\leq T$,
this is simply set equal to its in-sample observed value,
but for each point $t> T$, $i=1,\ldots,N$ different values are drawn. 
In Algorithm~2 we use
subscript $i$ and superscript $r$ to indicate quantities that correspond to draw $i$ 
for region $r$.  


\noindent \underline{Algorithm~2} {\em (Generating from the Gaussian ESN ensemble predictive distributions)}\\
\noindent
For each ESN configuration $\xivec^{1},\ldots,\xivec^{K}$ repeat the following:
\begin{itemize}
	\setlength{\itemindent}{0cm}
	\item[1.] For each of the five regional price series, compute $\hat{\varthetavec}^r$ using Algorithm~1.
	\item[2.] For $i=1,\ldots,N$, $t=T+1,\ldots,T+h_1$, and $r=1,\ldots,5$ do:
	\begin{itemize}
		\item[2.1] Construct $\xvec^r_{i,t}$ from previous series values $\{y^d_{i,s}\,;d=1,\dots,5,\,s=1,\ldots,t-1\}$
		\item[2.2] Compute $\hvec^r_{i,t}$ from $\{\hvec^r_{i,t-1},\xvec^r_{i,t}\}$ using the hidden state equation at~(1) in the main paper.
%		\item[2.3] Set $\bvec_{i,t}^r=\left[(\hvec_{i,t}^r)',((\hvec^r_{i,t})^{\circ 2})'\right]$
		\item[2.3] Draw $y_{i,t}^r$ from $\mathcal{N}(\hvec_{i,t}^r\hat{\betavec}_1^r+(\hvec_{i,t}^r)^{\circ 2}\hat{\betavec}_2^r,(\hat{\sigma}^2)^r)$ and store
		in an $(K N\times h_1 \times 5)$ array
	\end{itemize}
\end{itemize}

Algorithm~2 can be run in parallel 
over the $K$ configurations, while step~2.1 is undertaken using 
the
feature vector specification in Sec.~5.1 of the main paper. The algorithm produces
$KN$ draws from the joint ensemble forecast distribution of 
$(\bm{Y}_{\mbox{\tiny ALL},T+1},\ldots,\bm{Y}_{\mbox{\tiny ALL},T+h_1})$ of the 
Gaussian probabilistic 
ESN model. The $KN$ draws of each element in this vector
are from a marginal forecast distribution with ensemble density at~(5) of the main paper. 
In our empirical work we set $K=100$, $N=20$ and $h_1=24$, providing a total of $KN=2000$ draws for a vector of $5h_1=120$ future values. 
We run Algorithm~2 for each forecast origin in our evaluation period.
%Simply computing $\mbox{Price}^r_{i,t}=\exp(y^r_{i,t})-1001$
%converts these to draws from the forecast distribution of the
%nominal dollar-valued price processes.

\section{}\label{app:postST}
This appendix provides the MCMC sampler for drawing from
the posterior of $\varthetavec=\lbrace\betavec,\tau^2,\psi,\sigma^2\rbrace$ in the skew $t$ probabilistic 
ESN, augmented with 
the latent variables $\zetavec,\wvec$, for a given configuration $\xivec$.
The initial values for the parameters are $\sigma^2=c_0/(C_0+1)$ (prior mode), $\betavec=\nullvec$,  $\tau^2=0.1$,  $\psi=0$, $\zetavec=\nullvec$, $\wvec=\onevec$.

\noindent \underline{Algorithm~3} {\em (MCMC sampler for skew $t$ probabilistic ESN)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
	\setlength{\itemindent}{0.5cm}
	\item[1.] Generate from $\betavec|\{\varthetavec\setminus\betavec\},\wvec,\zetavec,X,\yvec$
	\item[2.] Generate from $p(\psi|\{\varthetavec\setminus\psi\},\wvec,\zetavec,X,\yvec)$
	\item[3.] Generate from $p(\sigma^2|\{\varthetavec\setminus\sigma^2\},\wvec,\zetavec,X,\yvec)$
	\item[4.] Generate from $p(\tau^2|\{\varthetavec\setminus\tau^2\},\wvec,\zetavec,X,\yvec)$
	\item[5.] For $t=1,\ldots,T$ generate from $p(\zeta_t|\varthetavec,w_{t},X_t,y_{t})$
	\item[6.] For $t=1,\ldots,T$ generate from $p(w_{t}|\varthetavec,\zeta_t,X,y_{t})$
\end{itemize}

\noindent 
All the conditional densities in steps~1 to 6 can be computed readily in 
closed form. In step~1, $\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$
where $\Sigma_{\beta}=(B_\xi(X)'W B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$, $\muvec_{\beta}=\Sigma_{\beta}(B_\xi(X)'W(\yvec-\psi\zetavec))/\sigma^2$
and $W=\mbox{diag}(\wvec)$ is a diagonal matrix of the latent variables.
At step~2,	$\psi\sim\mathcal{N}_1(\mu_{\psi},\sigma^2\sigma_{\psi})$,
where
$\sigma_{\psi}=(\zvec'W \zvec/\sigma^2+1/D_0)^{-1}$ and $\mu_{\psi}=\sigma_{\psi}(\zvec'W(\yvec-B_\xi(X)\betavec))/\sigma^2$. 
At step~3, 
$\sigma^2\sim\mathcal{IG}(c_k,C_k)$ with $C_k=C_0+\frac{1}{2}\left(\epsilonvec'W\epsilonvec+\frac{\psi^2}{D_0}\right)$, $\epsilon_{t}=y_{t}-b_{t}'\betavec-\psi \zeta_t$, $\epsilonvec=(\epsilon_{1},\ldots,\epsilon_{T})'$ and $c_k=c_0+\frac{1}{2}(T+1)$. At step~4, $\tau^2\sim\mathcal{IG}(b_k,B_k)$,
with $B_k=B_0+\frac{1}{2}\betavec'\betavec$ and $n_k=(b_0+p/2)$.
At step~5, $\zeta_t\sim\mathcal{TN}_{[0,\infty)}(a_{t},A/w_{t})$ with
$A=(1+\psi^2/\sigma^2)^{-1}$ and
$a_{t}=A\psi(y_{t}-B_\xi(X)'\betavec)/\sigma^2$. Finally, at step~6,
$w_{t}\sim\mathcal{G}(\nu/2+1,(\nu+\zeta_t^2+\epsilon_{t}^2/\sigma^2)/2)$,
where $\mathcal{G}$ denotes a gamma distribution.

%\begin{itemize}
%	\item[Step 1.] 
%	\[
%	\betavec|\lbrace\varthetavec\setminus\betavec\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta}),
%	\]
%	where $\Sigma_{\beta}=(B_\xi(X)'W B_\xi(X)/\sigma^2+1/\tau^2 I)^{-1}$, $\mu_{\beta}=\Sigma_{\beta}(B_\xi'W(\yvec-\psi\zetavec))/\sigma^2$
%	and $W=\mbox{diag}(w_1,\ldots,w_T)$ is a diagonal matrix of the latent variables.
%	\item[Step 2.]
%	\[
%	\psi|\lbrace\varthetavec\setminus\psi\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{N}_p(\muvec_{\psi},\sigma^2\Sigma_{\psi}),
%	\]
%	where $\Sigma_{\psi}=(z'W z/\sigma^2+1/D_0)^{-1}$ and $\mu_{\psi}=\Sigma_{\psi}(z'W(\yvec-B_\xi(X)\betavec))/\sigma^2$. 
%	\item[Step 3.] 
%	\[
%	\sigma^2|\lbrace\varthetavec\setminus\sigma^2\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{IG}(c_k,C_k),
%	\]
%	where $C_k=C_0+\frac{1}{2}\left(\epsilonvec'W\epsilonvec+\frac{\psi^2}{D_0}\right)$, $\epsilon_{t}=y_{t}-b_{t}'\betavec-\psi \zeta_t$, $\epsilonvec=(\epsilon_{1},\ldots,\epsilon_{T})'$ and $c_k=c_0+\frac{1}{2}(T+1)$.
%	\item[Step 4.] 
%	\[
%	\tau^2|\lbrace\varthetavec\setminus\tau^2\rbrace,\wvec,\zetavec,X,\yvec\sim\mathcal{IG}(b_k,B_k),
%	\]
%	where $B_k=B_0+\frac{1}{2}\betavec'\betavec$,  and $n_k=(b_0+p/2)$, as well as $p=\dim(\betavec)$.
%	%To perform a MH-step for the current value for $\tau^2$ we use the same Gaussian IWLS proposal for $log(\tau^2)$ as for the RNN and RNNC.
%	\item[Step 5.]  
%	\[
%	\zeta_t|\varthetavec,w_{t},\xvec_t,\yvec_{t}\sim\mathcal{TN}_{[0,\infty)}(a_{t},A/w_{t}),
%	\]
%	where 
%	\[
%	A=(1+\psi^2/\sigma^2)^{-1},\quad a_{t}=A\psi(y_{t}-B_\xi(X)'\betavec)/\sigma^2.
%	\]
%	\item[Step 6.] 
%	\[
%	w_{t}|\varthetavec,\zeta_t,\xvec_t,\yvec_{t}\sim\mathcal{G}\left(\frac{\nu}{2}+1,\frac{\nu+\zeta_t^2+\epsilon_{t}^2/\sigma^2}{2}\right).
%	\]
%%\end{itemize}
%After convergence, Algorithm~3 produces a Monte Carlo sample from the 
%augmented posterior distribution $\varthetavec,\wvec,\zetavec|X,\yvec$.

To simulate Monte Carlo draws from the ensemble forecast distribution at~(5) in the main paper,
Algorithm~2  is employed with minor adjustments. First, at step~1
the estimate $\hat{\varthetavec}^r$ is computed using Algorithm~3 above. 
Second, at step~2.3 
the iterate $y_{i,t}^r$ is drawn from a
$\mathcal{ST}(\hvec_{i,t}^r\hat{\betavec}_1+(\hvec_{i,t}^{r})^{\circ 2}
\hat{\betavec}_2^r,(\hat \omega^2)^r,\hat \alpha^r,\hat \nu^r)$ 
distribution. Here, at each sweep of Algorithm~3 draws of $\omega,\alpha$ are obtained from that of $\varthetavec$ as 
$\alpha=\psi/\sigma$ and $\omega=(\sigma^2+\psi^2)^{1/2}$, and 
the means of these draws computed to obtain $\hat \omega^r,\hat \alpha^r$. 

\section{}\label{app:postcop}
This appendix outlines the MCMC sampler for drawing from the 
posterior of $\varthetavec=\lbrace\betavec,\tau^2\rbrace$ in the deep copula model
for a given configuration $\xivec$. An algorithm for drawing from ensemble forecast distribution from the copula model is also given.

\noindent \underline{Algorithm~4} {\em (MCMC sampler for the deep copula)}\\
\noindent
Repeat the following steps sequentially:
\begin{itemize}
	\setlength{\itemindent}{0.5cm}
	\item[1.] Generate from $\betavec|\tau^2,X,\yvec$
	\item[2.] Generate from $\log(\tau^2)|\betavec,X,\yvec$
\end{itemize}
%\item[\textbf{Starting values}] For starting values we set $\betavec^{(0)}=\nullvec$,  $(\tau^2)^{(0)}=1$.

\noindent At step~1,
$\betavec\sim\mathcal{N}_p(\muvec_{\beta},\Sigma_{\beta})$, with
$\Sigma_{\beta}=(B_\xi(X)'B_\xi(X)+1/\tau^2 I)^{-1}$ and $\mu_{\beta}=\Sigma_{\beta}B_\xi(X)'\zvec$.  A Metropolis-Hastings step 
is used to generate $\upsilon=\log(\tau^2)$ at step~2, with
a Gaussian proposal with matching mode and curvature. Note that from
the conditional likelihood in Sec.~4.4, 
\begin{equation*}\label{eq:logFC:upsilon}
  \begin{aligned}
	  &l_{\upsilon}\equiv \log(p(\upsilon|X,\betavec,\yvec))\propto -\frac{\upsilon}{2}\left(\dim(\betavec)))-1\right)-\frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{b_{\tau^2}}\right)^{\tfrac{1}{2}}\\&
\quad\quad\quad\qquad\qquad\qquad\quad\;\,-\frac{1}{2}\sum_{i=1}^{n}\log(s_i^2)
-\frac{1}{2}\left(\zvec'(SS')^{-1}\zvec-2\betavec'B_\xi(X)'S^{-1}\zvec\right)\,.
  \end{aligned}
\end{equation*}
Approximating $l_{\upsilon}$ by a second order Taylor expansion around the current state $\upsilon^{(c)}$,
and taking the exponent, yields the proposal density $\ND\left(\mu_{\upsilon},\sigma_{\upsilon}^2\right)$ with
%\begin{equation*}\label{eq:param:proposal:tau2}
 $\mu_{\upsilon}=\sigma_{\upsilon}^2\frac{\partial l_{\upsilon}}{\partial\upsilon}+\upsilon$ and $\sigma_{\upsilon}^2=-1/\frac{\partial^2 l_{\upsilon}}{\partial\upsilon^2}.$
The derivatives in the proposal density for can be computed quickly in closed form
as
\begin{equation*}%\label{app:eq:deriv:tau2}
  \begin{aligned}
    \frac{\partial l_{\upsilon}}{\partial\upsilon}&= -\frac{1}{2}\left(\dim(\betavec)-1\right)+\frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{4b_{\tau^2}}\right)^{\tfrac{1}{2}}\\&\quad-\frac{1}{2}\sum_{i=1}^{n}\frac{1}{s_i^2}\frac{\partial}{\partial\upsilon}s_i^2 -\frac{1}{2}\left(\zvec'\left\lbrack\frac{\partial}{\partial\upsilon}(SS')^{-1}\right\rbrack\zvec-2\betavec'B_\xi(X)'\left\lbrack \frac{\partial}{\partial\upsilon}S^{-1}\right\rbrack\zvec\right)\\
    \frac{\partial^2 l_{\upsilon}}{\partial\upsilon^2}&= - \frac{1}{2\exp(\upsilon)}\betavec'\betavec-\left(\frac{\exp(\upsilon)}{16b_0}\right)^{\tfrac{1}{2}}-\frac{1}{2}\sum_{i=1}^{n}\left(\left\lbrack \frac{\partial}{\partial\upsilon}\frac{1}{s_i^2}\right\rbrack\frac{\partial}{\partial\upsilon}s_i^2+\frac{1}{s_i^2}\frac{\partial^2}{\partial\upsilon^2}s_i^2\right)\\&\quad -\frac{1}{2}\left(\zvec'\left\lbrack\frac{\partial^2}{\partial\upsilon^2}(SS')^{-1}\right\rbrack\zvec-2\betavec'B_\xi(X)'\left\lbrack \frac{\partial^2}{\partial\upsilon^2} S^{-1}\right\rbrack\zvec\right)\,.
  \end{aligned}
\end{equation*}
where the partial derivatives above are simple closed form expressions.

Algorithm~5 below is used to generate draws from the ensemble forecasting 
distribution at~(5) of the main paper for the deep copula model. It is an adjustment
of Algorithm~2 used for the probabilistic Gaussian ESN, with
similar super- and sub-script notation. Let 
$z_{i,t}^r$ denote the $i$th Monte Carlo draw of the (standardized)
pseudo-response in region $r\in\{1,\ldots,5\}$ at time $t$. For time points $t\leq T$, 
this is set equal to its in-sample value computed once as $z_{i,t}^r=\Phi_1^{-1}(F_Y(y^r_{t}))$. For time points $t>T$, $i=1,\ldots,N$ values
 are drawn for each ESN configuration.

\noindent \underline{Algorithm~5} {\em (Generating from the deep copula model ensemble predictive distributions)}\\
\noindent
For each ESN configuration $\xivec^{1},\ldots,\xivec^{K}$ repeat the following:
\begin{itemize}
	\setlength{\itemindent}{0cm}
	\item[1.] For each of the five regional price series, compute $\hat{\varthetavec}^r$ using Algorithm~4.
	\item[2.] For $t=1,\ldots,T$ and $r=1,\ldots,5$, compute $z_{i,t}^r=\Phi_1^{-1}(F_Y(y_{t}^r))$.
	\item[3.] For $i=1,\ldots,N$, $t=T+1,\ldots,T+h_1$, and $r=1,\ldots,5$ do:
	\begin{itemize}
		\item[3.1] Construct $\xvec^r_{i,t}$ from previous values $\{z^d_{i,s}\,;d=1,\dots,5,\,s=1,\ldots,t-1\}$.
		\item[3.2] Compute $\hvec^r_{i,t}$ from $\{\hvec^r_{i,t-1},\xvec^r_{i,t}\}$ using the hidden state equation at~(1).
		\item[3.3] Set $\bvec_{i,t}^r=\left[(\hvec_{i,t}^r)',((\hvec^r_{i,t})^{\circ 2})'\right]$ and compute $\psi_{i,t}^r=
		(1+\tau^2 \bvec_{i,t}^r(\bvec_{i,t}^r)')^{-1/2}$.
		\item[3.4] Draw $z_{i,t}^r$ from $\mathcal{N}(\psi_{i,t}^r\bvec_{i,t}^r \hat{\betavec}^r,(\psi_{i,t}^r)^2)$.
		\item[3.5] Set $y_{i,t}^r=F_Y^{-1}(\Phi_1(z_{i,t}^r))$ and store
		in an $(KN\times h_1 \times 5)$ array.
	\end{itemize}
\end{itemize}
Algorithm~5 can be run in parallel 
over the $K$ configurations, while step~3.1 is undertaken using 
the
feature vector specification in Sec.~5.1. The algorithm produces
$KN$ draws from the joint ensemble forecast distribution of 
$(\bm{Y}_{\mbox{\tiny ALL},T+1},\ldots,\bm{Y}_{\mbox{\tiny ALL},T+h_1})$ 
for the deep copula model. The $KN$ draws of each element in this $5h_1 \times 1$ vector
are from a marginal distribution with ensemble density of the
form at~(5) in the main paper. We use Algorithm~5 at each forecast origin in our evaluation period.
